Eigenmodes of the Laplacian on Hyperbolic Lattices

We examine a specific category of eigenfunctions of the lattice Laplacian on $\{p,q\}$-tessellations of the Poincar\'e disk that bear resemblance to plane waves in the continuum case. Our investigation reveals that the lattice eigenmodes deviate from the continuum solutions by a factor that depends solely on the local inclination of the vertex in relation to the wave's propagation direction. This allows us to compute certain eigenfunctions by numerical and analytical methods. For various special cases we find explicit exact eigenfunctions and their eigenvalues on the infinite lattice.

==> letter.tex <==
%=====================================================
% Main text of the letter
%=====================================================

\title{Eigenmodes of the Laplacian on Hyperbolic Lattices}
\author{Eric Petermann}
\email{eric.petermann@uni-wuerzburg.de}
\author{Haye Hinrichsen}
\email{haye.hinrichsen@uni-wuerzburg.de}
\affiliation{Institute for Theoretical Physics, Julius Maximilians University W\"urzburg, Am Hubland, 97074 Würzburg, Germany}

\begin{abstract}
We examine a specific category of eigenfunctions of the lattice Laplacian on $\{p,q\}$-tessellations of the Poincaré disk that bear resemblance to plane waves in the continuum case. Our investigation reveals that the lattice eigenmodes deviate from the continuum solutions by a factor that depends solely on the local inclination of the vertex in relation to the wave's propagation direction. This allows us to compute certain eigenfunctions by numerical and analytical methods. For various special cases we find explicit exact eigenfunctions and their eigenvalues on the infinite lattice.
\end{abstract}

\keywords{Hyperbolic Laplacian}
\maketitle

% Special definitions
\def\vec#1{\mathbf{#1}}

% %=====================================================
% \paragraph{Introduction:} \label{sec:Intro}
% %=====================================================

Formulating a consistent theory of quantum gravity remains one of the greatest challenges in modern physics. Such a theory is expected to not only describe the curvature of spacetime but also account for its potentially discrete nature at the Planck scale. To gain a deeper understanding of the interaction between curvature and discretization, quantum systems residing on tessellations of hyperbolic spaces with constant negative curvature~\cite{coxeter1957crystal} have emerged as a highly promising testing ground. In this context, various innovative experimental implementations, in particular photonic crystals~\cite{ozawa2019topological,kollar2019hyperbolic,yu2020topological} and electronic circuits on hyperbolic lattices~\cite{lee2018topolectrical,helbig2020generalized,dong2021topolectric,lenggenhager2021electric,lenggenhager2022simulating,chen2023hyperbolic,gluscevich2023dynamic}, are currently attracting significant attention.

These groundbreaking experiments have rekindled the interest in the fascinating mathematical properties of discretized hyperbolic spaces, particularly isometric tilings of the Poincaré disk. A significant milestone in this realm has been the development of hyperbolic band theory, drawing inspiration from solid-state physics~\cite{maciejko2021hyperbolic,boettcher2022crystallography,maciejko2022automorphic,ikeda2021hyperbolic,attar2022selberg,bzduvsek2022flat,mosseri2022aharonov,cheng2022band,zhang2023hyperbolic,liu2023higher,kollar2020line}. This theory combines the concept of Bloch waves~\cite{ashcroft2022solid} with group-theoretical ideas~\cite{katok1992fuchsian}, allowing one to describe specific categories of wave functions that exist within hyperbolic crystals.

From a mathematical point of view, the challenge of describing the band structure is closely intertwined with understanding the spectral properties of the discretized Laplace-Beltrami operator~\cite{boettcher2020quantum,bienias2022circuit}. However, unlike the Euclidean case where the eigenfunctions and eigenvalues of the lattice Laplacian can be easily computed, the eigenfunctions on hyperbolic lattices are significantly more intricate and generally cannot be expressed using closed formulas. The current band theory partially addresses this issue by assuming the existence of a translation subgroup on the lattice, which imposes certain limitations on possible lattice geometries. Nevertheless, a comprehensive classification of the eigenfunctions and eigenvalues of the hyperbolic lattice Laplacian remains elusive. Solving this problem would not only be valuable in the context of band theory but also hold profound implications for other fields, ranging from the AdS/CFT correspondence~\cite{maldacena1999large,witten1998anti,boyle2020conformal,asaduzzaman2020holography,brower2021lattice,basteiro2022towards} to applications in quantum information theory~\cite{ryu2006holographic,vidal2007entanglement,pastawski2015holographic,jahn2021holographic}.

As a further advancement in this direction, this Letter investigates a specific category of eigenfunctions of the Laplacian on infinite $\{p,q\}$-tilings of the Poincaré disk. These eigenfunctions on the lattice bear resemblance to plane waves in the continuum. To accomplish this, we introduce a novel geometric concept, referred to as the \textit{inclination} of a vertex. This concept plays a pivotal role in enabling us to provide exact solutions for a subset of points within the parameter space. Additionally, we propose two complementary numerical methods that facilitate the efficient computation of the eigenfunctions and their corresponding eigenvalues on the infinite lattice.

\vspace{2mm}
%=====================================================
\paragraph{Continuum Theory:} 
%=====================================================
%
Before we begin, let us provide a brief overview of the continuum description. The Poincaré disk serves as a conformal representation of the hyperbolic plane, characterized by a constant negative curvature. This representation is defined within an open unit disk, employing a conformal metric 
%
\begin{equation}
\text{d} s^2 \;=\; \frac{\text{d} z \text{d} \overline z}{(1-z \overline z)^2}\,,
\end{equation}
%
in which geodesic lines are represented by circular segments. The geodesic distance between two points
%
\begin{equation}
\text{d}(z,z') \;=\; \frac12\, \text{arcosh}\Bigl( 1+\frac{2|z-z'|^2}{(1-|z|^2)(1-|z'|^2)} \Bigr)
\end{equation}
%
is preserved under the isometries
%
\begin{equation}
\label{Isometry}
z \;\mapsto\; w(z)=e^{i\eta}\frac{a-z}{1-z \overline a}\,\,,
\end{equation}
%
where $\eta \in[0,2\pi)$ and $a\in\mathbb D$.
The Laplace-Beltrami operator on the Poincaré disk is given by
%
\begin{equation}
\label{LaplaceBeltrami}
\Delta_g \;=\; \frac{1}{\sqrt{g}}\partial_i\Bigl( \sqrt{g}\,g^{ij}\partial_j \Bigr) \;=\;4(1-z\overline z)^2\partial_z \partial_{\overline z}
\end{equation}
%
and its eigenvalue problem $\Delta_g \psi = -\lambda \psi$ is solved by~\cite{boettcher2020quantum}
%
\begin{equation}
\label{ContinuumPlaneWave}
\psi_{K}(z) = \left( \frac{1-|z|^2}{|1-z e^{-i\beta}|^2} \right)^{\frac12(1+ik)} \;\; \text{with} \;\;
\lambda=1+k^2,
\end{equation}
%
where $K=k e^{i\beta}$ is the generalized momentum. As explained in the supplement~\cite{noteSupplement}, these eigenfunctions can be regarded as plane waves emanating from an infinitely distant point located at the boundary $b=e^{i\beta} \in \partial \mathbb D$. These emitted waves travel along geodesic lines with perpendicular wave fronts referred to as \textit{horocycles}~\cite{anderson2005hyperbolic}.

In the context of AdS/CFT, a similar type of eigenvalue problem arises in the form of the Klein-Gordon equation $(\square-M^2)\psi = 0$ in Euclidean AdS$_2$ space. Here the primary focus lies on the \textit{exponential} eigenfunctions with imaginary momentum $k=\pm i \sqrt{1+M^2}$, as only then do the eigenmodes exhibit the required asymptotic behavior $\psi(z) \sim A(1-z \overline z)^{1-\Delta}+B(1-z \overline z)^{\Delta}$ for $|z|\to 1$. Here, $\Delta=\frac12(1+\sqrt{1+M^2})$ represents the scaling dimension of the boundary operator that is holographically dual to $\psi$\cite{ammon2015gauge}. Interestingly, these modes remain stable even for negative squared masses $M^2<0$ above the Breitenlohner-Freedman bound $M^2 \geq -1$\cite{breitenlohner1982stability,basteiro23breitenloher}.

As our results concern mainly the exponential modes, it will be convenient in the following to redefine $k$ by
%
\begin{equation}
\mu \;:=\;-\frac{1}{2}(1+ik)\,.
\end{equation}
%
Using this notation the continuum eigenfunction (\ref{ContinuumPlaneWave}) emitted from the source $b = e^{i \beta} \in \partial \mathbb D$ with eigenvalue $\lambda = -4\mu(\mu+1)$ and dimension $\Delta=\mu+1$ reads
%
\begin{equation}
\label{ContinuumPlaneWave2}
\psi_{\mu,b}(z) = \left( \frac{|b-z|^2}{1-|z|^2} \right)^{\mu}\,.
\end{equation}
%
Applying a Fourier transform in $\beta$, one obtains the corresponding radial eigenfunctions with $z=r e^{i \phi}$ in terms of associated Legendre functions:
%
\begin{equation}
\label{ContinuumRadialWave}
u_{\mu}^m(z) \;\propto\; e^{i m \phi} P^m_{\mu}\Bigl( \frac{1+r^2}{1-r^2} \Bigr)\,.
\end{equation}
%

\vspace{2mm}
%=====================================================
\paragraph{Lattice Laplacian:}
%=====================================================
Before we define the hyperbolic lattice Laplacian, let us briefly recall the Euclidean case. For instance, on a line with equidistant vertices at positions $x_j=jh$, the finite-difference operator
%
\begin{equation}
\Delta^{[h]} f(x_j) = \frac{1}{h^2}\bigl( f(x_{j+1})+f(x_{j-1})-2f(x_j) \bigr)
\end{equation}
%
is known to approximate the second derivative $f''(x_j)$. Generally, on a hypercubic lattice with vertices at $\vec{x}_j~\in~\mathbb{R}^n$ and spacing $h$, the discrete Laplacian $\Delta^{[h]}$ is given by
%
\begin{equation}
\label{EuclideanLatticeLaplacian}
\Delta^{[h]} f(\vec{x}_j) = \frac{1}{h^2}\left( A_{jk}-2d\delta_{jk} \right)f(\vec{x}_k),
\end{equation}
%
where $A_{jk}$ denotes the adjacency matrix which is $1$ if the nodes $j$ and $k$ are connected by an edge, and $0$ otherwise. The lattice Laplacian $\Delta^{[h]}$ is known to approximate the continuum Laplacian as $\Delta^{[h]} f(\vec{x}_j) = \nabla^2 f(\vec{x}_j) + \mathcal{O}(h)$.

Now, let us consider hyperbolic lattices on the Poincaré disk in the form of isometric $\{p,q\}$-tilings~\cite{coxeter1957crystal}. Such tilings consist of regular $p$-gons and vertices with coordination number $q$, satisfying the inequality $(p-2)(q-2)>4$, and can be easily generated using software packages such as~\cite{hypertiling}. Unlike Euclidean lattices, where the lattice spacing can be arbitrarily chosen, hyperbolic lattices have a fixed geodesic edge length.

Denoting the positions of the vertices on the Poincaré disk as $z_j\in\mathbb{D}$, the lattice Laplacian $\Delta^{\{p,q\}}$, which approximates the Laplace-Beltrami operator $\Delta_g$ in (\ref{LaplaceBeltrami}), is defined analogously to (\ref{EuclideanLatticeLaplacian}) as
%
\begin{equation}
\Delta^{\{p,q\}} f(z_j) = \frac{1}{\mathcal{N}}\left( A_{jk}-q\delta_{jk} \right)f(z_k),
\end{equation}
%
where the normalization is usually chosen as $\mathcal{N} = \frac{1}{4}q h^2$, with
%
\begin{equation}
\label{RadiusH}
h \;=\; \left(1-\frac{\sin^2 (\pi/q)}{\cos^2 (\pi/p)}\right)^{1/2},
\end{equation}
%
so that we recover $\Delta_g$ in the formal limit $h \to 0$~\cite{lenggenhager2022simulating}. The objective of this work is to find eigenvectors $\Psi_{\mu,b}(z_j)$ of the eigenvalue problem
%
\begin{equation}
\label{LatticeEigenvalueProblem}
\Delta^{\{p,q\}} \Psi_{\mu,b}(z_j) = -\Lambda_\mu \, \Psi_{\mu,b}(z_j)\,,
\end{equation}
%
which are analogous to the plane-wave eigenfunctions (\ref{ContinuumPlaneWave2}) in the continuum case.

\vspace{2mm}
%=====================================================
\paragraph{Special Solutions:} 
%=====================================================
%
In the Euclidean case, the continuum Laplacian $\Delta$ and its lattice counterpart $\Delta^{[h]}$ are known to have the \textit{same} eigenfunctions $\psi_{\vec k}(\vec x)=e^{i \vec k\cdot \vec x}$ for all $h>0$, although with different eigenvalues. In the hyperbolic case, this coincidence is generally absent, and the eigenfunctions on the lattice become highly nontrivial. Nonetheless, we have discovered specific values of $\mu$ where the coincidence still persists. More precisely, we have found that (\ref{LatticeEigenvalueProblem}) is solved by
%
\begin{equation}
\label{SpecialSolutions}
\Psi_{\mu,b}=\psi_{\mu,b} \qquad \qquad \text{for } \mu=0,1,\ldots,q-1
\end{equation}
%
with the eigenvalue
%
\begin{equation}
    \label{eq:GenZeroEigenvalues}
    \Lambda_\mu^{[0]}=\frac{q}{\mathcal N}\left( 1-P_\mu \Bigl( \tfrac{1+h^2}{1-h^2} \Bigr)\right)\,.
\end{equation}

\vspace{2mm}
%=====================================================
\paragraph{Main Hypothesis:} 
%=====================================================

An extensive numerical study for non-integer $\mu>0$ (not shown here) revealed that the lattice eigenfunctions analogous to plane waves differ only slightly from the continuum eigenfunctions~(\ref{ContinuumPlaneWave2}) and seem to exhibit the same exponential characteristics on large scales. This suggests that the lattice eigenfunctions $\Psi_{\mu,b}(z_j)$ differ from the continuum eigenfunctions $\psi_{\mu,b}(z_j)$ only by some \textit{correction factor} $\chi_j$, which is expected to be close to $1$ everywhere on the lattice:
%
\begin{equation}
\label{CorrectionFunction}
\Psi_{\mu,b}(z_j) \;=\; \psi_{\mu,b}(z_j)\, \chi_j\,.
\end{equation}
%
So far, this ansatz does not impose any restrictions. However, as a central hypothesis of this paper, we propose that the correction factor $\chi_j$ can only depend on the local environment surrounding $z_j$. Since all vertices on an infinite lattice are isometrically equivalent, we assume that, in~(\ref{CorrectionFunction}), the overall exponential behavior of the eigenmode is already factored out. Hence, we postulate that $\chi_j$ can solely depend on the direction in which the vertex "sees" the source $b=e^{i\beta}$ in relation to its nearest neighbors. In other words, it reflects how strongly the geodesic line originating from the source $b$ is locally tilted against the star of outgoing edges. For given $b$, we can thus define an angle $\alpha_j$ at each lattice site, as illustrated in the left panel of Fig.~\ref{fig:inclination}.
%
\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/inclination.png}
\caption{
\label{fig:inclination}
Left: $\{3,7\}$-tiling with a geodesic line (blue) originating at $b=1$ which crosses the vertex marked by the hollow circle. $\alpha$ is defined as the angle between the geodesic and the next edge in anti-clockwise direction. Right: Mapping the vertex conformally to the center (see text).
}
\end{figure}
Since $\alpha_j \in [0,2\pi/q)$, it will be convenient in the following to rescale it, defining the \textit{inclination}
%
\begin{equation}
\label{Inclination}
\tau_j \;:= \; \frac{q}{2\pi}\alpha_j \;\in\; [0,1)\,.
\end{equation}
%
As shown in the supplement, the inclination can be computed explicitly for each vertex at $z_j\in\mathbb D$ via the formula
%
\begin{equation}
\tau_j \;=\; \Bigl(\frac{1}{2\pi}\arg \Bigl[\Bigl( \frac{(1-b \overline z_j)(z'_j-z_j)}{(b-z_j)(1-z'_j\overline z_j)} \Bigr)^q\Bigr]\Bigr)\mod 1\,,
\end{equation}
%
where $z'_j$ denotes an arbitrarily selected nearest neighbor of $z_j$.

\vspace{2mm}
%=====================================================
\paragraph{Difference Equation for the Correction Function:} 
%=====================================================

With the above assumption that the factors $\chi_j$ depend solely on the inclination $\tau_j$, the primary task is to compute the \textit{correction function} $\chi(\tau)$. As demonstrated in the supplement, this leads to a non-local linear difference equation
%
\begin{equation}
\label{DifferenceEquation}
\sum_{n=0}^{q-1} R_n(\tau)\, \chi\bigl(\sigma_{n}(\tau)\bigr) \;=\; \bigl(q-\mathcal N \Lambda_\mu\bigr) \chi(\tau)
\end{equation}
%
holding for all $\tau \in [0,1)$, where
%
\begin{equation}
R_n(\tau) \;=\; \biggl( \frac{\bigl|1-h Z^{\tau+n}\bigr|^2}{1-h^2} \biggr)^{\mu}
\end{equation}
%
with $Z=e^{2\pi i/q}$ and
%
\begin{equation}
\sigma_{n}(\tau) \;=\; \Bigl(\frac{1}{2\pi} \arg \Bigl[ \Bigl( \frac{h-Z^{\tau+n}}{1-h Z^{\tau+n}} \Bigr)^q \Bigr]\Bigr) \mod 1\,.
\end{equation}
%
Analytically, it is straight-forward to verify that (\ref{DifferenceEquation}) is solved by $\chi(\tau)\equiv 1$ for $\mu=0,1,\ldots,q-1$, thus substantiating the special solutions in (\ref{SpecialSolutions}).

\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/numericaleigenmodes.png}
\caption{
\label{fig:chi}
Numerically determined correction function $\chi(\tau)$ on a $\{3,7\}$-lattice for various values of $\mu$ (see text).
}
\end{figure}


\vspace{2mm}
%=====================================================
\paragraph{Numerical Iteration Scheme:}
%=====================================================
The difference equation~(\ref{DifferenceEquation}) can be regarded as an eigenvalue problem for $\chi(\tau)$, and it turns out that the eigenfunctions with the largest eigenvalue correspond to the plane-wave solutions we aim to determine (for $\mu\geq0$). This suggests a simple numerical iteration scheme. For this, we first divide the domain of the inclination $\tau\in[0,1)$ into $T$ equidistant bins labeled by the index $t=0,\ldots,T-1$, thereby discretizing the inclination function $\chi(\tau)$ by a vector $\vec X$ with the components $X_t \simeq \chi(t/T)$. Setting
%
\begin{align}
R_{n,t}    &:= R_n(t/T)\\
s_{n,t} &:= \lfloor T \sigma_n(t/T)\rfloor
\end{align}
%
and initializing $X^{[0]}_t:=1$, we iterate $\vec X^{[k]}\mapsto \vec X^{[k+1]}$ via
%
\begin{align}
&Y_t \;:=\; \sum_{n=0}^{q-1} R_{n,t} X^{[k]}_{s_{n,t}}  \quad (t=0\ldots,T-1)
\\
&\eta \;:=\; \frac{1}{T}\sum_{t=0}^{T-1} |Y_t|
\\
&\vec X^{[k+1]} \;:=\; {\vec Y}/{\eta}
\end{align}
%
in a loop until $\vec X^{[k]}$ becomes stationary. The corresponding eigenvalue can then be estimated by $\Lambda_\mu \approx \frac{1}{\mathcal N}(q-\eta)$.

Fig.\ref{fig:chi} shows the numerically determined approximation of the correction function $\chi(\tau)$ for various values of $\mu$. As anticipated, the algorithm reproduces $\chi\equiv 1$ for $\mu=0,1,\ldots,q-1$. For $\mu=q,q+1,\ldots,2q-1$, we find that $\chi(\tau)$ can be fitted by $1+a \cos(2\pi \tau)$ within machine precision, while for all other values of $\mu$, especially non-integer ones, more Fourier components seem to be involved. For negative values of $\mu$, the algorithm still converges, but it produces irregular solutions with a fractal structure reminiscent of Weierstrass functions. In all cases, we can use (\ref{CorrectionFunction}) to compute the full eigenfunction $\Psi_{\mu,b}(z_j)$ and directly verify its validity on the infinite tiling.


\vspace{2mm}
%=====================================================
\paragraph{Analytical Solution:}
%=====================================================
%
The numerical results propose representing $\chi(\tau)$ as a Fourier series
%
\begin{equation}
\label{FourierAnsatz}
\chi(\tau) \;=\; \sum_{k=-\infty}^{+\infty} \gamma_k \; e^{2\pi i \tau k}
\end{equation}
%
with $\gamma_0:=1$. As shown in the supplement, this converts the difference equation (\ref{DifferenceEquation}) into an eigenvalue problem for the coefficients $\gamma_k$ of the form
%
\begin{equation}
\label{GammaEVProblem}
\sum_{k=-\infty}^{\infty} B_{j,k}\,\gamma_k \;=\; (q-\mathcal N \Lambda_\mu) \gamma_j\,.
\end{equation}
%
Here, the infinite-dimensional matrix $B$ is defined by
%
\begin{equation}
B_{j,k} = \frac{q \,(-1)^{qj}\,h^{q|j-k|}}{(1-h^2)^\mu}
\begin{cases}
\binom{\mu-qk}{\mu-qj}F_{qj,-qk}(h^2) & \text{ if } j\geq k \\
\binom{\mu+qk}{\mu+qj}F_{-qj,qk}(h^2) & \text{ if } j< k
\end{cases}
\end{equation}
%
where $F_{a,b}(\xi)={}_2F_1\bigl(a-\mu,\,b-\mu;\,1-a-b;\,\xi\bigr)$
and $\binom{a}{b}=\tfrac{\Gamma(1+a)}{\Gamma(1+b)\Gamma(1+a-b)}$. Note that the matrix $B_{j,k}$ is transposed under the substitution $\mu \to -1-\mu$, implying the crucial symmetry of the eigenvalues
%
\begin{equation}
\Lambda_\mu =\Lambda_{-1-\mu}\,.
\end{equation}
%
Interestingly, for $\mu \in \mathbb N$ the matrix $B$ possesses a block structure. More specifically, if $qs \leq \mu < q(s+1)$ with $s~\in~\mathbb N$, this permits us to solve the eigenvalue problem only within the central block matrix where $j,k\in{-s,\ldots,+s}$. Consequently, for $\mu\in\mathbb N$, the Fourier series (\ref{FourierAnsatz}) contains only $2s+1$ terms. This observation is one of the main results of this work.

The block structure enables us to compute various special cases exactly. For instance, for $\mu=0,1,\ldots q-1$, we simply reproduce the special case in Eqs. (\ref{SpecialSolutions})-(\ref{eq:GenZeroEigenvalues}), where the lattice and continuum eigenfunctions coincide. For $\mu=q,\ldots,2q-1$, we find an explicit exact solution for the lattice eigenfunction, provided in the supplement.

Eq.~(\ref{GammaEVProblem}) is also beneficial for non-integer $\mu>0$, as we can approximate the solution numerically by truncating the matrix $B$ at a certain size, resulting in highly accurate numerical solutions.

\vspace{2mm}
%=====================================================
\paragraph{Radial Lattice Eigenfunctions:}
%=====================================================
%
Having calculated the plane-wave lattice eigenfunctions originating from $b = e^{i\beta} \in \partial \mathbb D$, the corresponding radially symmetric solutions analogous to $u_{\mu}^m(z)$ in Eq. (\ref{ContinuumRadialWave}) can be obtained through a simple Fourier transformation in the angle $\beta$:
%
\begin{equation}
U_{\mu}^m(z_i)\;=\;\frac{1}{2\pi}\int_0^{2\pi} e^{i m \beta}\,\Psi_{\mu,e^{i\beta}}(z_i)
\,.
\end{equation}
%
In this context, a straightforward calculation (see supplement) leads to the following explicit expression in terms of the coefficients $\gamma_k$:
%
\begin{equation}
\begin{split}
U_{\mu}^m(z_j) &=\frac{1}{(1-|z_j|^2)^\mu}\,
\sum_{k=-\infty}^\infty \gamma_k
\left[ \frac{z_j-z'_j}{h (1-z'_j \bar z_j)} \right]^{qk} \times \\
&
\times
% \binom{\mu-q k}{\mu-m}\,{}_2 F_1\bigl(-\mu-qk,\;-\mu+m;\;1+m-qk;\;|z_j|^2\bigr)
\begin{cases}
z_j^{m-q k}\binom{\mu-q k}{m-q k}\, F_{m,-qk}(|z_j|^2) & \text{ if } m \geq q k \\
\overline z_j^{q k-m}\binom{\mu+q k}{q k-m}\,  F_{-m,qk}(|z_j|^2)  & \text{ if } m < q k \\
\end{cases}
\end{split}
\end{equation}


\vspace{2mm}
%=====================================================
\paragraph{Conclusions:} 
%=====================================================
%
In this Letter, we introduced a method for computing specific eigenfunctions of the hyperbolic lattice Laplacian on the Poincaré disk which are analogous to plane waves in the continuum case. Our approach hinges on the assumption that such eigenfunctions deviate from the continuum solutions by a correction factor $\chi(\tau)$, which depends solely on the so-called 'inclination' $\tau$ of the respective vertex relative to the propagation direction of the wave.

We provided a numerical iteration scheme alongside an analytical method that allows us to determine the correction function $\chi(\tau)$ for given lattice parameters ${p,q}$ and the exponent $\mu$. Furthermore, we demonstrated that for $\mu\in\mathbb N$, this correction function incorporates only a finite number of Fourier modes, which allows various special cases to be solved exactly.

It is noteworthy that our method functions for any ${p,q}$ and does not rely on edge pairing and the existence of a Fuchsian translation subgroup. Moreover, once $\chi(\tau)$ and the eigenvalue $\Lambda_\mu$ are determined, it promptly allows the calculation of the eigenfunction on the entire infinite lattice without cutoff.

Despite these advances, many questions remain open. In the current study, we focused on (unnormalizable) exponential modes with $\mu>0$, corresponding to imaginary momenta $k=i(1+2\mu)$. As hinted by the numerical results, the form of the eigenfunctions for $\mu<0$ is significantly more irregular, and the interpretation of these findings is not yet clear. It would also be intriguing to study oscillatory modes with real momenta. Preliminary tests suggest that the proposed methods remain partially functional, but this requires further detailed exploration. Additionally, we analyzed only a specific eigenvalue of the difference function leading to a plane-wave analog, so far neglecting many other possible solutions. Finally, the correlation between our results and hyperbolic band theory and Fuchsian symmetry is still to be clarified.

%=====================================================
\begin{acknowledgments}
\paragraph{Acknowledgements:} We are grateful to J.~Erdmenger for fruitful discussions.
\end{acknowledgments}
%=====================================================

